Stronger, Cheaper and Demonstration-Free Log Parsing with LLMs

Log parsing, the process of converting raw log messages into structured formats, is an important initial step for automated analysis of logs of large-scale software systems. Traditional log parsers often rely on heuristics or handcrafted features, which may not generalize well across diverse log sources or require extensive model tuning. Recently, some log parsers have utilized powerful generative capabilities of large language models (LLMs). However, they heavily rely on demonstration examples, resulting in substantial overhead in LLM invocations. To address these issues, we propose LogBatcher, a cost-effective LLM-based log parser that requires no training process or labeled data. To leverage latent characteristics of log data and reduce the overhead, we divide logs into several partitions through clustering. Then we perform a cache matching process to match logs with previously parsed log templates. Finally, we provide LLMs with better prompt context specialized for log parsing by batching a group of logs from each partition. We have conducted experiments on 16 public log datasets and the results show that LogBatcher is effective and efficient for log parsing.

==> sections/related-work.tex <==
Log parsing has recently become an active research topic due to its practicality~\cite{he2017drain, du2016spell, le2023log}. So far, log parsers can be classified into three categories: syntax-based, semantics-based, and LLM-based log parsers.

\textbf{Syntax-based Log Parsers} Syntax-based log parsers utilize manually designed features to extract log templates. Syntax-based log parsers are generally unsupervised and typically employ three techniques: \textit{(1) Frequent patterns mining:} Some log parsers~\cite{dai2020logram, vaarandi2015logcluster, nagappan2010abstracting} extract log templates by identifying the constant parts of log messages through the mining of frequent patterns, specifically n-grams.\textit{(2) Clustering:} Logs that belong to the same template exhibit similarities. Consequently, some methods~\cite{fu2009execution,  tang2011logsig, shima2016length} employ clustering techniques to group logs and extract the constant portions of log messages for log parsing.\textit{(3) Heuristics:}  Heuristics-based log parsers~\cite{jiang2008abstracting, du2016spell, he2017drain} leverage unique characteristics from log messages to extract common templates efficiently.

\textbf{Semantic-based Log Parsers} 
Semantic-based log parsers generally leverage semantic information from labeled data, formulating log parsing as a token classification problem. UniParser~\cite{liu2022uniparser} is a unified log parser designed for heterogeneous log data, trained with labeled data from multiple log sources to capture common patterns of templates and parameters. Although effective, UniParser requires a significant amount of labeled data for training and relies on handcrafted rules to split raw log messages into tokens, which may not always be feasible in practice. LogPPT~\cite{le2023log} introduces a novel paradigm for log parsing, employing template-free prompt-tuning to fine-tune the pre-trained language model, RoBERTa. By mining the semantic information contained within the pre-trained model and fine-tuning it with a minimal amount of log data, LogPPT achieves high performance in terms of accuracy and robustness.

\textbf{LLM-based Log Parsers} Recently, many log parsing methods have started to rely on large language models (LLMs) due to their extensive pre-trained knowledge of code and logs. \cite{le2023evaluation} validated the potential of LLMs in log parsing and achieved promising results. DivLog~\cite{xu2024divlog} and LILAC~\cite{jiang2023lilac} enhance the performance of large models by selecting demosntrations from labeled log data and utilizing the in-context learning capabilities of LLMs. These methods are sensitive to the quantity and coverage of labeled logs and incur LLM inference overhead. Lemur~\cite{zhang2024lemur} invokes LLM to merge generated similar templates, improving the accuracy of log parsing groupings. However, it requires extensive hyperparameter tuning for specific datasets.

Compared to other parsers, \tool does not require heuristic rules, handcrafted features, training process, or labeled data. In other words, \tool can be directly applied to log parsing in efficiently and effectively.

%for any system, achieving both robust and effective results.







